DreamFit: Garment-Centric Human Generation via a Lightweight Anything-Dressing Encoder

Diffusion models for garment-centric human generation from text or image prompts have garnered emerging attention for their great application potential. However, existing methods often face a dilemma: lightweight approaches, such as adapters, are prone to generate inconsistent textures; while finetune-based methods involve high training costs and struggle to maintain the generalization capabilities of pretrained diffusion models, limiting their performance across diverse scenarios. To address these challenges, we propose DreamFit, which incorporates a lightweight Anything-Dressing Encoder specifically tailored for the garment-centric human generation. DreamFit has three key advantages: (1) \textbf{Lightweight training}: with the proposed adaptive attention and LoRA modules, DreamFit significantly minimizes the model complexity to 83.4M trainable parameters. (2)\textbf{Anything-Dressing}: Our model generalizes surprisingly well to a wide range of (non-)garments, creative styles, and prompt instructions, consistently delivering high-quality results across diverse scenarios. (3) \textbf{Plug-and-play}: DreamFit is engineered for smooth integration with any community control plugins for diffusion models, ensuring easy compatibility and minimizing adoption barriers. To further enhance generation quality, DreamFit leverages pretrained large multi-modal models (LMMs) to enrich the prompt with fine-grained garment descriptions, thereby reducing the prompt gap between training and inference. We conduct comprehensive experiments on both $768 \times 512$ high-resolution benchmarks and in-the-wild images. DreamFit surpasses all existing methods, highlighting its state-of-the-art capabilities of garment-centric human generation.

==> sec/abstract.tex <==
\begin{abstract}


Diffusion models for garment-centric human generation from text or image prompts have garnered emerging attention for their great application potential.
However, existing methods often face a dilemma: lightweight approaches, such as adapters, can result in inconsistent textures; while finetune-based methods involve high training costs and struggle to maintain the generalization capabilities of pretrained diffusion models, limiting their performance across diverse scenarios. To address these challenges, we propose DreamFit, which incorporates a lightweight Anything-Dressing Encoder specifically tailored for the garment-centric human generation. 
DreamFit has three key advantages: (1) \textbf{Lightweight training}: with the proposed adaptive attention and LoRA modules, DreamFit significantly minimizes the model complexity to 83.4M trainable parameters. (2)\textbf{Anything-Dressing}: Our model generalizes surprisingly well to a wide range of (non-)garments, creative styles, and prompt instructions, consistently delivering high-quality results across diverse scenarios. (3) \textbf{Plug-and-play}: DreamFit is engineered for smooth integration with any community control plugins for diffusion models, ensuring easy compatibility and minimizing adoption barriers.
To further enhance generation quality, DreamFit leverages pretrained large multi-modal models (LMMs) to enrich the prompt with fine-grained descriptions of the garment, thereby reducing the prompt gap between training and inference. We conduct comprehensive experiments both on $768 \times 512$ high-resolution benchmarks and in-the-wild images. DreamFit surpasses all existing methods, highlighting its state-of-the-art capabilities of garment-centric human generation.

\end{abstract}

==> sec/experiment.tex <==
\section{Experiment}

\subsection{Datasets}
To train Dreamfit, we collected approximately 500,000 garment-person image pairs from the internet and captioned them using large multi-modal models.
For model evaluation, we introduce two garment-centric human generation benchmarks derived from public dataset and the internet.  The open benchmark is constructed using a subset of VITON-HD \cite{choi2021viton} and DressCode \cite{morelli2022dress} test sets. Specifically, we handpicked 200 diverse garments from these datasets encompassing various styles, colors, shapes, and textures. Each garment is associated with refined prompts generated through large multi-modal models. 
In addition to the open benchmark, we further developed a more challenging internal benchmark. To build the internal benchmark, we manually gathered 200 reference images from the internet, including garments with intricate textures and backgrounds, and non-garment images featuring animals, fruits, and patterns. This benchmark is designed to evaluate the robustness and generalization capability of the model across diverse reference image types.
% Experiments are conducted under a resolution of $768 \times 512$., 
% \zxj{ need update the detail of dataset, anything to add?}
% our proprietary e-commerce dataset contains 57,239 training pairs and 5,219 testing pairs of front-view full-body person and in-store garment images, and 200,931 training pairs and 29,198 testing pairs of multiple front-view images of the same full body.

% \zxj{Note,some package are not allowed }

\begin{figure*}
  \centering
  \includegraphics[width=0.9\textwidth]{AnonymousSubmission/LaTeX/fig/more_result_3.pdf}
  \caption{Plug-and-play results of DreamFit, our method can seamlessly integrate with community conditional control plugins.}
  \label{fig:more_result}
\end{figure*}

\subsection{Implementation Details}

The denoising UNet is initialized with the weights of SD1.5 and we use CLIP ViT-L/14 \cite{radford2021learning} as the text encoder. Our model was trained on paired images with a resolution of $768 \times 512$. We initialized the LoRA layers in the same manner as described in \cite{hu2021lora}, with the LoRA rank set to 64. The training was conducted on 8 A800 (40G) GPUs for 90k steps, with a batch size of 4 per GPU. We utilized the AdamW optimizer with a fixed learning rate of 1e-4. 
To validate scalability, we also initialized the denoising UNet as SDXL and trained the model on 8 A100 (80G) GPUs for 90k steps with the same batch size. Thanks to the efficient model design, acceleration techniques such as FSDP or Deepspeed were not required for training. 
During inference, we use CogVLM \cite{wang2023cogvlm} to rewrite and refine the user input text. We use DDIM \cite{song2020denoising} sampler with 50 steps and set guidance scale $w$ to 7.5. 

% \linente{Should we mention that we have trained a version of the SDXL model?}
% \zxj{You can just mention what you did on xl.}
\subsection{Baselines}
We selected four state-of-the-art methods, including StableGarment \cite{wang2024stablegarment}, MagicClothing \cite{chen2024magic}, IMAGDress \cite{shen2024imagdressing}, and IP-Adapter \cite{ye2023ip}. 
We directly use their released pretrained models for comparison. All experiments are conducted with a resolution of $768 \times 512$.

\subsection{Qualitative Results}
The qualitative comparison is illustrated in Figure~\ref{fig:comparsion}. The results demonstrate the superiority of our DreamFit over other baselines. Firstly, our method exhibits better texture and text consistency. Existing lightweight approaches, such as IP-Adapter, lose text and texture consistency when faced with reference images containing complex details. While finetune-based methods like StableGarment, MagicClothing, and IMAGDress surpass IP-Adapter significantly, they still struggle to generate human images with fine-grained features that highly match the text prompts.
Secondly, images generated by baselines generally exhibit issues such as blurriness (IMAGDress) and incorrect body proportions (third row of StableGarment column). In contrast, our method achieves the best quality and realism. To show the model's excellent compatibility, we provide additional results showcasing DreamFit integrated with community plugins in Figure~\ref{fig:more_result}.
% Firstly, our method employs Lightweight Anything-Dressing Encoder, which results in better texture consistency compared to the baseline. Secondly, as our approach ewrite the user input text based on reference images, it achieves greater effect， showcasing the effectiveness of our method.


\subsection{Quantitative Results}
% \zxj{remove all of "stable" in the score}
\noindent\textbf{Metric.} We quantitatively measure the generated results from three aspects: CLIP-T for text consistency, CLIP-I \cite{hessel2021clipscore} for texture consistency, and Aesthetic score(AS) \cite{schuhmann2022laion} for generation quality.
CLIP-T computes the cosine similarity between the generated images and the input prompts within the CLIP feature space to quantify text consistency. CLIP-I measures the similarity between the generated images and the reference images to assess texture consistency. The Aesthetic Score (AS) is derived from an aesthetic model trained on LAION-5B \cite{schuhmann2022laion}. 
To mitigate the impact of randomness, we generate five results for each reference image, and use all of them for metric computation.
 
% These metrics are designed to measure the stability and consistency of the generated images with respect to the reference images.


\noindent\textbf{Evaluation.} We conducted experiments using both open and internal benchmarks to assess the performance of our model against baselines. The quantitative results are reported in Tab. \ref{quantitative-results-table}.
Our DreamFit consistently outperforms all baselines across all metrics and benchmarks, demonstrating its ability to generate results with superior text and texture consistency, and overall generation quality. 
Furthermore, compared with fully finetune-based methods, e.g., StableGarment, IMAGDress, DreamFit has the fewest trainable parameters while achieving the best performance. This indicates that DreamFit is more parameter-efficient and robust.

% including lightweight IPAdapter, StableGarment, MagicClothing, and IMAGDress. The evaluation was performed on multiple aspects of image generation, focusing on the alignment of generated images with their corresponding textual and visual prompts.


% \zxj{ maybe one more metric to fill the space?}
\begin{table*}[ht]
    \centering
    \begin{tabular}{l|c|ccc|ccc}
        \toprule
        {{Method} & {Trainable Parameters} & \multicolumn{3}{c}{Open Benchmark} & \multicolumn{3}{c}{Internal Benchmark} \\ 
        \cline{3-8}
        & & CLIP-T$\uparrow$ & CLIP-I$\uparrow$ & AS$\uparrow$ & CLIP-T$\uparrow$ & CLIP-I$\uparrow$ & AS$\uparrow$ \\ 
        \midrule
        IP-Adapter & 22M & 0.257 & 0.631 & 4.667 & 0.135 & 0.422 & 2.634 \\ 
        StableGarment & 859M & 0.263 & 0.654 & 4.877 & 0.275 & 0.629 & 5.238 \\ 
        MagicClothing & 875M & 0.285 & 0.641 & 5.007 & 0.320 & 0.583 & 5.462 \\ 
        IMAGDress & 875M & 0.300 & 0.720 & 4.867 & 0.290 & 0.632 & 5.204 \\ 
        Ours & 83.4M & \textbf{0.328} & \textbf{0.740} & \textbf{5.414} & \textbf{0.334} & \textbf{0.687} & \textbf{5.516} \\ 
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
    \caption{Quantitative comparison of different methods on three metrics for both open and internal benchmarks.}
    \label{quantitative-results-table}
\end{table*}

% \noindent The table above presents the quantitative results of our method compared to several baselines. Our model, with significantly fewer trainable parameters, achieves superior performance in most metrics across both open and internal evaluations, demonstrating the efficiency and effectiveness of our approach.


\subsection{Ablation Study}

\begin{figure}
  \centering
  \includegraphics[width=1.0\hsize]{AnonymousSubmission/LaTeX/fig/ablation_network.pdf}
  % \vspace{-6mm}
  \caption{Qualitative results of the ablation study on network components.}
   % \vspace{-4mm}
  \label{fig:ablation_components}
\end{figure}

\subsubsection{Effectiveness of Network Components}

To evaluate the impact of different network components on the final performance, we conducted an ablation study comparing various model configurations. We experiment with three setups: finetuning the entire Anything-Dressing Encoder (finetuning), only optimizing parameters in LoRA layers (only LoRA), only optimizing parameters of adapters in adaptive attentions (only Adapter). The results are summarized in the Tab. \ref{table:ablation-study1} and the qualitative results are shown in Figure \ref{fig:ablation_components}.

Despite having the highest number of trainable parameters, finetuning the entire Anything-Dressing Encoder exhibited subpar performance on text and texture consistency. We conjecture this is because finetuning can compromise the model's pre-trained prior, leading to a decline of its feature extraction capability. While the "only LoRA" and "only Adapter" configurations showed better texture consistency than finetuning, they performed inadequately for generation quality. In contrast, our DreamFit, which combines and optimizes both LoRA and Adapter, achieves superior results across all metrics, underscoring its efficiency and efficacy.

\begin{figure}
  \centering
  \includegraphics[width=1.0\hsize]{AnonymousSubmission/LaTeX/fig/ablation2.pdf}
  % \vspace{-6mm}
  \caption{Qualitative results of the ablation study on text prompts.}
   % \vspace{-4mm}
  \label{fig:ablation_text}
\end{figure}

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{3pt} % Adjust column separation
\renewcommand{\arraystretch}{0.9} % Adjust row separation
\begin{tabular}{l c c c c}
  \toprule
  {Method} & \makecell{Trainable \\Parameters} & {CLIP-T$\uparrow$} & {CLIP-I$\uparrow$} & {AS$\uparrow$} \\
  \midrule
  Finetuning        & 875M  & 0.322 & 0.622 & \textbf{5.534} \\
  Only LoRA              & 66M   & 0.322 & 0.686 & 5.250 \\
  Only Adapter           & 17.4M & 0.310 & 0.679 & 5.230 \\
  Ours                   & 83.4M & \textbf{0.334} & \textbf{0.687} & 5.516 \\
  \bottomrule
\end{tabular}
\caption{Quantitative results of the ablation study on network
components}
\vspace{-5mm}
\label{table:ablation-study1}
\end{table}

\begin{table}[t]
\small
\centering
\begin{tabular}{l c c c}
  \toprule
  {Method} & {CLIP-I $\uparrow$} & {AS$\uparrow$} & {Human Study$\uparrow$} \\
  \midrule
  Fixed text       & 0.588 & 5.283 & 0.03 \\
  Simple text     & 0.663 & 5.186 & 0.10 \\
   Ours        & \textbf{0.687} & \textbf{5.516} & \textbf{0.87} \\
  \bottomrule
\end{tabular}
\caption{Quantitative comparison of different text prompt configurations.}
\label{table:ablation-study2}
\vspace{-5mm}
\end{table}

\subsubsection{Impact of Text Prompts}

To further explore the influence of text prompts, we conducted experiments with three different types of text inputs: (1) a fixed text prompt (fix text), (2) a simple text prompt (simple text) for simulating user input, and (3) text prompts rewritten by LMMs (Ours). The qualitative and quantitative results for each configuration are shown in Figure. \ref{fig:ablation_text} and Tab. \ref{table:ablation-study2}.

The results demonstrate that text prompts rewritten by large multi-modal models yield superior quality outputs across all metrics, including notably higher scores in human study evaluations. This underscores the efficacy of incorporating advanced LMMs to enhance prompts with detailed descriptions of reference images, thereby narrowing the gap between training and inference prompts and boosting the quality and realism of the generated images.

\section{Conclusion}

In this paper, we introduced \textbf{DreamFit}, a novel garment-centric human image generation framework designed to address the inefficiencies and limitations of existing methods. By leveraging a lightweight, plug-and-play Anything-Dressing Encoder based on LoRA layers, DreamFit significantly streamlines model complexity and memory usage, facilitating more efficient and scalable training procedures. Our approach integrates large multi-modal models into the inference process, effectively reducing the domain gap between training and inference text prompts and enhancing the overall quality and consistency of the generated images.
Extensive experiments conducted on open and internal benchmarks demonstrate that DreamFit not only achieves state-of-the-art performance but also exhibits superior generalization capabilities across diverse scenarios. 
\vspace{6mm}
% \textbf{Limitation}
% \textbf{furture work}
% \zxj{Do we need clarify limitation and furture work?}

==> sec/introduction.tex <==

\section{Introduction}

Garment-centric human generation aims to synthesize high-quality images of stylized humans based on diverse combinations of text and image prompts, with a focus on accurately depicting the given garment details, as shown in Figure~\ref{fig:teaser}. 
This technology has gained significant traction in industries such as creative advertising and fashion design and has consequently sparked active exploration in the academic community \cite{wang2024stablegarment, chen2024magic}.


However, this task faces two critical challenges: the resource-intensive process of full model fine-tuning and the domain gaps between training and inference text prompts. 
Specifically, finetune-based methods like StableGarment\cite{wang2024stablegarment} rely on a full copy of diffusion UNet as the garment encoder, namely the ``ReferenceNet'', which consumes high GPU memory and becomes intractable when scaling up from SD1.5\cite{SDInpainting} to SDXL\cite{podell2023sdxl}. Moreover, directly fine-tuning the entire UNet is parameter inefficient, which also increases training times, and is prone to destroying the pretrained priors. As a result, the extracted garment feature is less descriptive, making it difficult to fully preserve the texture details (Figure~\ref{fig:teaser} Bottom). Alternatively, some lightweight  methods \cite{ye2023ip, mou2024t2i} attempt to bypass the bulky ReferenceNet by directly mapping image features into the CLIP \cite{radford2021learning} latent space to control the generation through cross attention. Although these approaches can accelerate the training process, they tend to overlook crucial image details. Therefore, the trade-off between training efficiency and preservation of visual details is a significant problem when generating human images from garment prompts.

\begin{figure}
  \centering
  \includegraphics[width=1.0\hsize]{AnonymousSubmission/LaTeX/fig/motivation.pdf}
  \vspace{-6mm}
  \caption{Performance comparison between baselines and our DreamFit. The circle size represents the number of trainable parameters, with larger circles indicating a higher parameter count. Higher CLIP-I and CLIP-T scores signify better alignment between the generated results and text descriptions. Our method not only achieves the best performance but also maintains much fewer training parameters.}
   \vspace{-4mm}
  \label{fig:motivation}
\end{figure}

Another challenge is the domain gap between the text prompts for training and inference. To fully leverage the rich prior of the text-to-image diffusion model, the training text prompts generated by Large Multi-modal Models (LMMs) are typically precise and comprehensive \cite{choi2024improving}. Yet during testing, users often resort to simplified text due to the difficulty of manually creating rich prompts. Such a gap further complicates the garment-centric generation process.


To address these challenges, we introduce DreamFit, a novel framework specifically designed for garment-centric human generation. DreamFit leverages a lightweight, plug-and-play Anything-Dressing Encoder, which consists of trainable LoRA layers and a denoising UNet, avoiding finetuning a full copy of the UNet\cite{hu2024animate}. Our model focuses on efficient output modulation, achieving better alignment with specific domain standards with minimal computation. 
% \zfw{Missing LoRA in this paragraph.}
Furthermore, to bridge the gap between training and inference text prompts, DreamFit incorporates LMMs into the inference pipeline. This integration minimizes discrepancies, ensuring that the generated images maintain high fidelity and consistent quality across a variety of scenarios.

As shown in Figure \ref{fig:motivation}, DreamFit beats all baselines at CLIP-I and CLIP-T metrics, showing the best text and texture consistency of generation results even with much fewer trainable parameters (83.4M v.s. 875M full model fine-tuning). Our main contributions are summarized as follows:

\begin{figure*}
  \centering
    \captionsetup{type=figure}
    \includegraphics[width=1.0\textwidth]{AnonymousSubmission/LaTeX/fig/architecture.pdf}
  \caption{
Overview of DreamFit. Our method constructs an Anything-Dressing Encoder utilizing LoRA layers. The reference image features are extracted by the Anything-Dressing Encoder and then passed into the denoising UNet via adaptive attention.  Furthermore, we incorporate large multi-modal models into the inference process to reduce text prompt gap between training and inference stages.
  } 
  \label{fig:architecture}
\vspace{-5mm}
\end{figure*}

\begin{itemize}
    \item We propose \textbf{DreamFit}, a comprehensive framework tailored for garment-centric human generation, enabled by a lightweight and plug-and-play Anything-Dressing Encoder. Our model addresses the inefficiencies and limitations of existing methods, particularly in the areas of model fine-tuning and computational efficiency.
    \item We integrate large multi-modal models into the inference pipeline that effectively reduces the prompt gap between training and testing, enhancing the overall quality and fidelity of the generated images.
    \item Extensive experiments on open and internal benchmarks at the resolution of $768 \times 512$

    verify the superiority of DreamFit, demonstrating state-of-the-art performance and robust generalization across diverse scenarios.\footnote{{Our code and model will be released upon acceptance.}}
\end{itemize}



==> sec/method.tex <==
\section{Methodology}


\subsection{Preliminary}
\label{sec:SD}
Stable Diffusion is a text conditioned latent diffusion model~\cite{rombach2022high}. Given a latent feature $z_0$ encoded from the input image by a VAE~\cite{kingma2013auto}, the forward diffusion process is firstly performed by adding noise according to a predefined noise scheduler $\alpha_t$~\cite{ho2020denoising}:
\begin{equation}
q(z_t|z_0) = \mathcal{N}(z_t; \sqrt{\alpha_t}z_0, (1 - \alpha_t)I).
\end{equation}
Then to reverse the diffusion process to generate new images, an noise estimator $\epsilon_\theta(\cdot)$ parameterized by an UNet is learned to predict the forward added noise $\epsilon$ with the objective function as follows:
\begin{equation}
\mathcal{L}_\text{dm} = \mathbb{E}_{\boldsymbol{z}_{0}, \boldsymbol{\epsilon}, \boldsymbol{c}_{t}, t}
\left[ ||\epsilon - \epsilon_\theta (z_t, t, c_t)||^2 \right],
\end{equation}
where $c_t$ is the text condition associated with the image latent $z$, and $D$ refers to the training set. In the Stable Diffusion model, each block of the UNet consists of cross-attention and self-attention layers. The cross-attention layer facilitates attention between the image feature query and the text condition embedding, while the self-attention layer operates within the image feature space.

\subsection{DreamFit}

The overall architecture of DreamFit is shown in Figure \ref{fig:architecture}. 
Our model consists of two main components: a frozen denoising UNet with pretrained stable diffusion weights, and a set of trainable LoRA layers that efficiently interact with the denoising UNet. 
DreamFit takes as input a reference garment image and a text prompt that describes the detail of the \textbf{output} image.
The text prompt features, extracted by a frozen text encoder, are integrated into the denoising UNet via a cross-attention mechanism. The features of the reference image are extracted by a lightweight Anything-Dressing Encoder, which is activated by turning on the LoRA layers in the denoising UNet. Once the LoRA layers are turned off, the lightweight Anything-Dressing Encoder reverts to the denoising UNet. The extracted reference features are then integrated into the denoising UNet through an adaptive self-attention mechanism. After multiple rounds of denoising, the denoising UNet generates an image that closely aligns with the reference image and text prompt. We elaborate the anything-dressing encoder and the adaptive attention in the following sections.

\textbf{Lightweight Anything-Dressing Encoder.}
The core concept of our model is that the pretrained diffusion model possesses extensive prior knowledge, making it a robust feature extractor. However, the features extracted by the pretrained diffusion model cannot be directly utilized for conditional generation tasks. To address this, we employ LoRA layers to adjust the pretrained diffusion model, allowing it to adapt to the task of feature extraction while preserving its strong prior knowledge. Specifically, we incorporated the LoRA layers into the linear and convolutional layers of the denoising UNet, modifying the forward pass as follows:
\begin{equation}
    h = \phi (x) + I(x)* \Delta W (x)
\end{equation}

\begin{equation}
    I(x) = \left\{\begin{matrix}
    0  & x=z_t,\\
    1  & x=c_i, \\
    \end{matrix}\right.
\end{equation}
Here, $\phi$ denotes the linear or convolutional layers in the denoising UNet. $\Delta W$ denotes the added LoRA, which consists of two linear layers, i.e., $\Delta W=B A$, where $B \in \mathbb{R}^{d \times r}, A \in \mathbb{R}^{r \times k}$. $z_t$ and $c_i$ represent the latent noise and the features extracted from the reference image, respectively. $I(x)$ denotes a signal function, acting as a gate that only open when the input is the reference features $c_i$.
By this approach, we only need to train the parameters of the LoRA layers (approximately 60M) to transform the denoising UNet into the lightweight Anything-Dressing Encoder, endowing it with strong feature extraction and generalization capabilities. 

\textbf{Adaptive attention.}
As shown in Figure \ref{fig:architecture}, the reference image features are integrated into the denoising UNet through adaptive attention. During training, the weights of the denoising UNet are frozen, which can hinder the pretrained attention module from effectively capturing the relationship between reference image features and the latent noise. Inspired by the adapter mechanism \cite{ye2023ip}, we introduced two trainable linear projection layers $\mathbf{W}_{k}^{\prime}$, $\mathbf{W}_{v}^{\prime}$, into the adaptive attention. These layers act as adapters to align the reference image features with latent noise. After applying cross-attention mechanisms, we add the cross-attention output to the self-attention output. The formulation of adaptive attention is:
\begin{equation}
\mathbf{z}_{t}^{\text {new }}=\operatorname{Softmax}\left(\frac{\mathbf{Q} \mathbf{K}^{\top}}{\sqrt{d}}\right) \mathbf{V}+\operatorname{Softmax}\left(\frac{\mathbf{Q}\left(\mathbf{K}^{\prime}\right)^{\top}}{\sqrt{d}}\right) \mathbf{V}^{\prime}
\end{equation}
where  
$\mathbf{Q}=\mathbf{z}_{t} \mathbf{W}_{q}, \mathbf{K}=\boldsymbol{z}_{t} \mathbf{W}_{k}, \mathbf{V}=\boldsymbol{z}_{t} \mathbf{W}_{v}, \mathbf{K}^{\prime}=\boldsymbol{c}_{i} \mathbf{W}_{k}^{\prime}, \mathbf{V}^{\prime}=\boldsymbol{c}_{i} \mathbf{W}_{v}^{\prime}$, and $\mathbf{W}_{q}, \mathbf{W}_{k}, \mathbf{W}_{v}$ are frozen linear projection layers in the denoising UNet. To accelerate the attention coverage, we initialize the  $\mathbf{W}_{k}^{\prime}$, $\mathbf{W}_{v}^{\prime}$ with $\mathbf{W}_{k}$, $\mathbf{W}_{v}$.
The trainable parameters of the adapters in the adaptive attention are only about 17M. This allows us to seamlessly and lightweightly inject the reference image features into the denoising UNet, resulting in synthesized images that are highly consistent with the reference image.

\begin{figure*}
  \centering
  \includegraphics[width=0.8\textwidth]{AnonymousSubmission/LaTeX/fig/compare2.pdf}
  \caption{Qualitative comparison on the open and internal benchmarks. DreamFit demonstrates a distinct advantage in handling complex patterns and text. Please zoom in for more details.}
  \label{fig:comparsion}
\end{figure*}

\textbf{Training and inference}
During the training phase, we exclusively optimize the LoRA layers and the trainable adapters in the adaptive attention, totaling approximately 83M parameters. Dreamfit is trained on a dataset containing image-text pairs, with the text generated by Language Model Models (LMMs), such as CogVLM \cite{wang2023cogvlm} and LLaVA1.5 \cite{liu2024improved}. To fully leverage the rich prior of the text-to-image diffusion model \cite{choi2024improving}, we prepare comprehensive captions for each image (e.g., "woman wears a long-sleeved polo shirt..."). The training objective remains consistent with the original diffusion model:
\begin{equation}
L_{\text {LDM }}=\mathbb{E}_{\boldsymbol{z}_{0}, \boldsymbol{\epsilon}, \boldsymbol{c}_{t}, \boldsymbol{c}_{i}, t}\left\|\boldsymbol{\epsilon}-\boldsymbol{\epsilon}_{\theta}\left(\boldsymbol{z}_{t}, \boldsymbol{c}_{t}, \boldsymbol{c}_{i}, t\right)\right\|^{2}
\end{equation}
During the inference phase, users are expected to input a reference image and a text description related to the desired output image. However, users often struggle to accurately describe fine-grained details in images and tend to provide simple text, leading to a domain gap between user input text and training text. This gap can result in decreased consistency and quality of the generated images. To address this challenge, we propose utilizing LMMs to rewrite the user input text based on the reference images. This approach enriches the text prompt with fine-grained descriptions of the garment, thereby reducing the prompt gap between training and inference. We denote the rewritten text as ${c}_{t}^{\prime}$. Then, we apply classifier-free guidance \cite{ho2022classifier} during the denoising process:
\begin{equation}
\hat{\boldsymbol{\epsilon}}_{\theta}\left(\boldsymbol{z}_{t}, \boldsymbol{c}_{t}^{\prime}, \boldsymbol{c}_{i}, t\right)=w \boldsymbol{\epsilon}_{\theta}\left(\boldsymbol{z}_{t}, \boldsymbol{c}_{t}^{\prime}, \boldsymbol{c}_{i}, t\right)+(1-w) \boldsymbol{\epsilon}_{\theta}\left(\boldsymbol{z}_{t}, t\right)
\end{equation}

% \zxj{write the meaning of symbol,make preliminary and this equation consistency}


==> sec/related_work.tex <==
\section{Related work}

human generation has witnessed rapid advancements, particularly with the emergence of controllable text-to-image generation technologies. . Existing methods in this field often concentrate on either enhancing lightweight efficiency or enhancing texture consistency. However, these approaches struggle to balance the trade-offs between computational requirements and image quality.

Lightweight methods like \cite{hu2021lora, ye2023ip, mou2024t2i, zhang2023adding, ruiz2023dreambooth, chen2024anydoor,liu2024ada,han2024face,yang2024lora,li2024swiftdiffusion,xing2024tryon} have been proposed as lightweight approaches to achieve controllable human generation. These methods typically align image features with text features, using a combination of text and visual prompts to guide the generation process. T2I-adapter \cite{mou2024t2i} designed a series of convolutional layers to downsample and extract the reference image features, which are then fed into the denoising UNet via residual connections. IP-Adapter \cite{ye2023ip} introduces a sophisticated decoupled cross-attention mechanism to integrate image features into the denoising UNet. Although these methods excel in lightweight design, they often struggle to maintain high texture consistency, especially in intricate garment details. In contrast, our method not only retains the same level of lightweight efficiency but also ensures significantly improved texture consistency.

% 网络设计了一系列卷积层来讲参考图片进行下采样，下采样后的图像特征通过残差连接的方式被引入到去噪UNet中
Additionally, several  methods \cite{zhu2023tryondiffusion,morelli2023ladi,zhang2023warpdiffusionefficientdiffusionmodel,wang2024mv,xu2024ootdiffusion,zhu2024m,kim2023stableviton,zhang2024mmtryon,hu2024animate,cui2023street} aiming for better texture consistency have chosen to utilize the UNet from Stable Diffusion as the image encoder to capture image prompt features. StableGarment \cite{wang2024stablegarment} finetunes a trainable copy of denoising UNet as the garment encoder and incorporates garment features using additive self-attention. MagicClothing \cite{chen2024magic} proposes joint classifier-free guidance to obtain a trade-off between garment features and text prompts. While these approaches, which require extensive finetuning of pretrained models such as those based on Stable Diffusion, yield commendable results in terms of quality, they come with significant drawbacks. These methods are resource-intensive, demanding significant memory resources and exhibiting sluggish training procedures, thus limiting their scalability for real-world applications.
% \textbf{Huamn AIGC comparision }\zxj{for note not real title leave for ente}
% \textbf{summary}

Our work builds on these developments by leveraging frozen large diffusion models (LDMs) for garment-centric human image synthesis. We introduce a lightweight, plug-and-play Anything-Dressing Encoder that addresses the inefficiencies and limitations of existing methods, offering a scalable and flexible solution for garment-centric human image synthesis.


%Human Generation has been a rapidly advancing field, especially with the advent of text-to-image (T2I) generation and editing technologies. However, existing methods often struggle with inconsistencies in garment textures and the high computational costs associated with fine-tuning large models. Various strategies have been proposed to address these challenges by introducing conditional controls and efficient model adaptations.
%For instance, methods like LoRA \cite{hu2021lora} and IP-Adapter \cite{ye2023ipadapter} aim to enhance T2I diffusion models by conditioning them on high-level semantic cues derived from reference images. These approaches typically use a combination of text and visual prompts to guide the generation process, offering more control over the final output. However, these methods often require significant computational resources, particularly when fine-tuning large models such as those based on Stable Diffusion.

%In response to these challenges, alternative approaches like ControlNet \cite{zhang2023controlnet} and T2I Adapter \cite{mou2024t2iadapter} have been developed. These methods introduce additional conditional encoding modules—such as edges, depth, and human poses—to better control the diffusion process in T2I models. While these techniques offer improved control, they still face issues related to memory consumption and training efficiency.

%Recent works, such as Uni-ControlNet \cite{zhao2024unicontrolnet}, propose unified frameworks that handle various conditional controls within a single model, thereby reducing computational costs. Similarly, methods like MasaCtrl \cite{cao2023masactrl} and InstructPix2Pix \cite{brooks2023instructpix2pix} leverage self-attention transformations and additional input channels to achieve consistent and flexible image generation without the need for extensive retraining.

%Our work builds upon these advances by leveraging the capabilities of frozen large diffusion models (LDMs) in the context of garment-centric human image synthesis and editing. By introducing a lightweight, plug-and-play garment encoder, we aim to address the inefficiencies and limitations of existing methods, offering a more scalable and flexible solution for person image synthesis.

